Towards Calibration Enhanced Network by Inverse Adversarial Attack

Test automation has become increasingly important as the complexity of both design and content in Human Machine Interface (HMI) software continues to grow. Current standard practice uses Optical Character Recognition (OCR) techniques to automatically extract textual information from HMI screens for validation. At present, one of the key challenges faced during the automation of HMI screen validation is the noise handling for the OCR models. In this paper, we propose to utilize adversarial training techniques to enhance OCR models in HMI testing scenarios. More specifically, we design a new adversarial attack objective for OCR models to discover the decision boundaries in the context of HMI testing. We then adopt adversarial training to optimize the decision boundaries towards a more robust and accurate OCR model. In addition, we also built an HMI screen dataset based on real-world requirements and applied multiple types of perturbation onto the clean HMI dataset to provide a more complete coverage for the potential scenarios. We conduct experiments to demonstrate how using adversarial training techniques yields more robust OCR models against various kinds of noises, while still maintaining high OCR model accuracy. Further experiments even demonstrate that the adversarial training models exhibit a certain degree of robustness against perturbations from other patterns.

==> misc/cvpr2025/preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> misc/cvpr2025/sec/0_abstract.tex <==
\begin{abstract}
%The robustness of a model against perturbation has been deeply explored for many years.
   %The issue of model calibration has been studied for many years. A well calibrated model is very important for the reliable predictions in some safety tasks, for example, face authentication and auto-driving system. While adversarial examples can reveal the overconfidence issues of models under slightly data distribution shifts (e.g., noise perturbation) to some extent, the other side of miscalibration—underconfidence—has rarely been addressed. In this paper, we innovatively propose a new task, termed as  Inverse Adversarial Attack, to highlight potential underconfidence issues in models. Furthermore, we introduce the examples generated by Inverse Adversarial Attack in the training process to enhance the model's calibration. Unlike adversarial training that focus on amending overconfidence adversarial examples, this inverse adversarial training aims to adjust underconfidence cases during training. Ultimately, by combining adversarial training and inverse adversarial training, we can achieve a model that excels in both robustness and calibration.
   Model calibration has been a focus of study for many years, as a well-calibrated model is crucial for reliable predictions in safety-critical tasks, such as face authentication and autonomous driving systems.While adversarial examples can reveal overconfidence issues in models under slight perturbations, the opposite issue—underconfidence—has rarely been addressed. In this paper, we introduce a novel task, termed Inverse Adversarial Attack (IAA), to highlight potential underconfidence issues in models. Additionally, we incorporate examples generated by IAA during the training process to improve model calibration. Unlike traditional adversarial training, which primarily addresses overconfident adversarial examples, inverse adversarial training focuses on adjusting underconfident cases. Ultimately, by combining adversarial and inverse adversarial training, we can develop a model that excels in both robustness and calibration.
\end{abstract}

\textbf{Keyword:}
Model Calibration, Underconfidence Examples, Inverse Adversarial Attack.

%dunning kruger effect表明 认知是从不知道自己不知道到知道自己不知道进发的，而在知道自己不知道这个问题上大多数文章都讨论的是边界清晰的OOD,然而heavy perturbation下的image的over confidence问题鲜有人探讨。本文提出了一个新的问题，即 如何调整模型 让它的输出不会over confidence的无视perturbation 。 而perturbation与confidence的关系是很主观的事情。。。。

%比如自动驾驶系统在高躁环境下（如 雨天） 不能对自己的结果over confidence
%于是我们提出在training 过程中加入一个term 会根据加入的perturbation 降低他的output的confidence
%然而随机噪声过于低效，为了精准的找到这样的（over confidence）example 我们从inverse adversarial attack的角度 来寻找这样的inverse adversarial example，最后提出inverse adversarial training来降低模型 over confidence的问题


%treat the noise as a kind of distrubution shift of the data , how to measure the influnce of this shift to the model.
%we try to train a model that can reflect the distribution shift of the input data




%2024-10-24
%under-confidence -> over performing
%如果错判结果（flase positive）severe 那么overconfidence是我们要关注租的问题
%如果false positive 严重 那么under confidence 是我们更要解决的问题
%class specific confidence training
%confidence equalizer

==> misc/cvpr2025/sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

%神经网络在分类时会输出“置信度”分数和预测结果。理想情况下，这些分数应该与真实正确性的可能性相匹配。例如，如果我们将 80% 的置信度分配给 100 个样本，那么我们就会期望 80% 样本的预测实际上是正确的。如果是这样，我们说模型是经过校准的。 

%我们最终目的是校准模型calibrated，让模型不会overconfidence or lack confidence

%模型可能会过度自信地做出错误的预测，特别是在面对分布偏移或未见过的数据时。

%很多model uncertainty的文章仅仅考虑clear image的校准问题，而从未讨论过分布偏移（noise）情况下的模型校准问题

%本文中不考虑OOD的case，仅仅讨论模型对于perturbation/noise的分布偏移而产生的uncertainty的表现



%我们希望模型不仅能给出分类的置信度得分，还希望模型能给出的置信度能恰好等于模型真实的预测准确率。因为分类问题中模型的最终输出是类别，而置信度是模型对判断为该类别的信心程度，已经是对模型给出的此次决策的可信程度的判断了）

%因为accuracy和confidence最好一致，即高accuracy对应高confidence，而随着noise增加 accuracy降低的同时confidence并未降低。这样的矛盾会使得model产生危险的判断。所以我们设计了一个loss 加入random noise之后 如果分类正确，则mmc越高越好，如果分类错误则mmc越低越好。

%这个noise如果使用adversarial technique获得，

%metric 宏观： accuracy plot和mmc plot的差距
%metric 微观： class_correct(f(X)) * mmc(f(X))
% metric loss=nllloss(log((1+x)/2)) 
% x = class_correct(f(X)) * mmc(f(X))
%adv： 分类错误  mmc高
%iad： 分类正确 mmc低

%与AA的区别
%我们的IAA的目的是寻找找出分类正确但是confidence过低的case， 或者找出分类错误但是confidence过高的case。后者与AA类似，但是AA没有考虑到分类结果与confidence的关系，我们想找出的是体现了model分类结果与confidence的contradiction的case。

%与AT的区别
%在训练中，我们考虑的是找出分类正确但是mmc过低的case提高其mmc， 找出分类错误但是mmc过高的case降低其mmc。后一个case与对抗训练类似，然而对抗训练的目的是修改分类结果，即提高label对应的confidence。而我们的训练方向是作用于mmc，目的为使得mmc与分类正确与否相关，最终在统计意义上使得accuracy与confidence一致


%由于目的不同，AA是为了低噪环境下提高model的鲁棒性，所以其epsilon一般设置较低（<0.3）,而我们是为了让accuracy与confidence相统一，这一般出现在高噪环境下（如图），所以epsilon一般设置较高（>0.5）


%AT 
\if 0
As accuracy on clean input is an opposite property to robustness, the control of ``robustness'' of the model can help increase the accuracy on benign inputs.

In some cases, as the noise/perturbation increases, the accuracy decreases, however, the mean maximum confidence is still very high. That means the model is overconfident in its wrong predictions. In other words, the model lacks resilience against \textbf{data distribution shifts}.
For a good model, high confidence should come with high accuracy. 
In this paper, we address the issue of determining the appropriate level of confidence a model should exhibit when it encounters a perturbed input.



We show an example of MNIST classification problem in~\cref{IAA:fig:cover} to illustrate the existence of IAE. As shown in (a), the clear image can be correctly predicted by the ResNet50 DNN classifier with $99.9\%$ confidence. After adding a Random Noise (b) with perturbation $\epsilon=0.8$, the prediction confidence of label 3 decreases to $1.1\%$. 
The IAE in (c) has a significantly heavier perturbation than Random Noise (b). However, the model correctly predicts the input as $3$ and the prediction confidence is counter-intuitively high.
%
This example shows the phenomenon that a well-trained DNN model may be over-confident with some noise patterns, which contain confused information for human beings.

In that case, we point out a statement that the confidence should decrease as the perturbation increases, which aligns with human beings' perceptions.
%
However, human is subjective. Everyone has different explanations for the problem of how confidence should decrease upon the perturbation level.
%
As a result, we just propose a general framework to bridge the gap between human beings and AI models.
%
Our proposed framework is not limited to any specific metric; however, to validate the effectiveness of the framework in our experiments, we designed a particular function tailored to a specific task or metric.

%一个训练好的模型对于分布偏移是否具有足够的抵抗性
%随着噪声增加， accuracy降低而mmc依旧很高、这中矛盾reveal plain trained model的不足
%即对数据的分布偏移没有抵抗力

%AI 法官用model    
%self driving 情况下 天气 雨天  雨水 perturbed camera， model should not be so confidence to its result at that senario
\fi

%---------------------------
\begin{figure}[t]
\centering
        \centering
        \includegraphics[width=1\linewidth]{./figure/cover/cover.pdf}
        \caption{An image of a \textbf{Samoyed} dog from the ImageNet dataset, predicted by a pretrained ResNet50 DNN classifier, demonstrates the presence of the Inverse Adversarial Example. (a) The clear input is correctly classified as \textbf{Samoyed} with a confidence of $40.1\%$. (b) The Adversarial Example, with a perturbation of $\epsilon=0.03$, is misclassified as \textbf{Eskimo} with a confidence of $76\%$. (c) The Inverse Adversarial Example, also with a perturbation of $\epsilon=0.03$, is correctly classified as \textbf{Samoyed}, but with a very low confidence of $2.3\%$. The prediction confidence distributions for the corresponding inputs are shown at the bottom.}
        %\caption{An image of \textbf{Samoyed} dog in ImageNet dataset predicted by a pretrained ResNet50 DNN classifier shows the existence of the Inverse Adversarial Example. (a) Clear input is correctly predicted as \textbf{Samoyed} with confidence of $40.1\%$. (b) Adversarial Example with perturbation $\epsilon=0.03$ is wrongly predicted as \textbf{Eskimo} with confidence of $76\%$. (c) Inverse Adversarial Example with perturbation $\epsilon=0.03$ is correctly predicted as \textbf{Samoyed}, but with very limited confidence of $2.3\%$. The prediction confidence distributions of corresponding input are listed on bottom.}    
\label{IAA:fig:cover}
% \vspace{-4mm}
\end{figure}
%---------------------------


% %---------------------------
% \begin{figure}[t]
% \centering
%         \centering
%         \includegraphics[width=1\linewidth]{./figure/IAEcompare/uncalibration.pdf}
%         \caption{The comparison results between accuracy and confidence with different perturbation $\epsilon$ on CIFAR10 dataset with a well-trained ResNet18 DNN classifier.}    
% \label{IAT:fig:cover}
% % \vspace{-4mm}
% \end{figure}
% %---------------------------


%模型的calibration 问题已经被研究很多年了，然而模型在data distribution shifting情况下的calibration并未完全的explored。虽然adversarial examples可以一定程度上揭示模型在data distribution shift（e.g. noise perturbation）的情况下存在的overconfidence问题，un-calibration的另外一面：underconfidence却很少被提及。所以本文创新性的提出了一种新的calibration inverse adversarial example （CIAE）来揭示模型可能存在的under confidence问题。并且在training中引入新的term来纠正model的uncalibration。与传统adversarial training不同的是，这种calibration training旨在修正confidence而非accuracy。这种方式可以使CT的功能专注于calibration的强化，进而与强化robustness的传统AT在功能上区分开来。最终，结合CT和AT我们可以获得一个robustness和calibrated表现均良好的model



 
%Calibration 是很重要的性质，而robustness enhancement的AT可以一定程度上解决overconfidence的问题，因为AE在错判的前提下，经常具有很高的confidence。甚至有的work以confidence作为loss的一项来寻找AE【CCAT】
%然而。由于misCalibration包含两个方面，而adversarial training只专注于将overconfidence的case矫正（错判-》对判），但是忽视了underconfidence的case。所以本文与ae相反，着重寻找iae，来进一步提高model在data shifting中的Calibration。
%-------------------------------------- 
%-----------   motivation   ----------- 
%-------------------------------------- 
Calibration is a critical property for ensuring reliable prediction in safety-related tasks, \eg, face recognition, commercial judgment \cite{buchel2022deep,aastebro2007calibration}, diagnosis \cite{gallaher2004impact,caruana2015intelligible} and self-driving \cite{wu2021way,bojarski2016end}. 
%
In many real-world tasks, accuracy alone is not the only measure of model quality, as the true label of an input case is not known in advance. Therefore, confidence is also considered alongside the model's output to determine how to proceed with decisions and whether additional procedures are needed \cite{wang2023calibration}. Deploying uncalibrated models can be risky: if the output is overconfident, it is likely to mislead subsequent decisions. Conversely, if the output is underconfident, the system may cast unnecessary doubt, leading to excessive interventions and higher costs due to expert involvement, ultimately reducing efficiency.
%

Adversarial Attacks (AA) typically generate examples that cause networks to become overconfident in their predictions \cite{teixeira2023reducing}. Thus, adversarial training (AT) for robustness enhancement can partially address the overconfidence issue by integrating adversarial examples (AEs) into the training process, as these examples often exhibit high confidence despite incorrect predictions.
Some studies even incorporate prediction confidence as a term in the loss function to address the overconfidence of AEs \cite{stutz2020confidence}.

However, since miscalibration involves both overconfidence and underconfidence, adversarial training primarily focuses on correcting overconfident cases (incorrect to correct predictions) while neglecting underconfident cases. In contrast, this study introduces a novel task that generates examples correctly predicted but with limited confidence, termed ``Inverse Adversarial Attack'' (IAA). The corresponding examples are ``Inverse Adversarial Examples'' (IAEs). They can thus be leveraged to expose underconfidence issues into training process, termed Inverse Adversarial Training (IAT), and further enhance model calibration against tiny perturbations.

%An example from ImageNet dataset \cite{deng2009imagenet} is listed in \cref{IAA:fig:cover}. It is easy to see that AE can provide a wrong prediction result and the corresponding confidence is even higher than the clear input. Such examples result in an overconfidence issue of the target model. In terms of IAE, it holds the correct prediction but with a very limited confidence ($2.3\%$). It reveals the underconfidence problem of a well-trained model. 
An example from the ImageNet dataset \cite{deng2009imagenet} is presented in \cref{IAA:fig:cover}. It is evident that AE produces an incorrect prediction with a confidence level even higher than that of the clear input, highlighting the overconfidence issue in the target model. On the other hand, IAE provides the correct prediction but with very limited confidence ($2.3\%$), exposing the underconfidence problem in a well-trained model.

%-------------------------------------- 
%-----------   contribution   ----------- 
%-------------------------------------- 
Generally, our contributions are as follow:
\begin{itemize}
\item We propose a novel task, \ie, Inverse Adversarial Attack, which focuses on generating underconfidence examples, referred to as Inverse Adversarial Examples. These examples satisfy two conditions: they are \textbf{correctly predicted} by the model but with \textbf{limited confidence}.
\item We introduce two cross-entropy loss terms to represent the two conditions of underconfidence examples, and combine them using a positive weight parameter to construct the final loss function $\mathcal{L}$. And we also mathematically prove that, by minimizing the loss function we can ensure the IAEs can truely satisfy the two conditions of underconfidence examples.
\item Inspired by Adversarial Training, we introduce the IAEs as an augmentation in training process, and propose Inverse Adversarial Training which aim to defend the underconfidence attack.
\item The experiments demonstrate the effectiveness of IAA in exposing a model's underconfidence issues, while IAT effectively defends against such attacks. The combination of AT and IAT is shown to be practical, providing a model that is both robust and well-calibrated.
\end{itemize}
%cover image: 
%clear image: confidence bar of 10 classes
%IAE: confidence bar of 10 classes

==> misc/cvpr2025/sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> misc/cvpr2025/sec/2_related_work.tex <==
\section{Related Works}
\label{sec:relatedwork}
\subsection{Calibration Methods}

% Generally, there are two way to achieve a model's calibration, including post-hoc calibration and calibration training.
% %
% Post-hoc calibration tends to calibrate the output confidence of a model, serving as a post processing. The advantage is that there is no need to update or retrain the exist model.
% Zadrozny \etal \cite{zadrozny2001obtaining} first utilized histogram binning to obtain calibrated probability estimates from decision tree and naive Bayesian classifiers. After that, they introduced the isotonic regression to achieve calibration \cite{zadrozny2002transforming}. Other than that, a more efficient and low-cost post-hoc method is Platt scaling \cite{platt1999probabilistic} and its single-parameter extension Temperature Scaling has many extension version\cite{mozafari2018attended,kull2019beyond,ding2021local}.
%
% In terms of calibration training method,
% Zhang \etal \cite{zhang2017mixup} introduced a mixup regularization to generate simple linear relationship between training examples. 
% Tomani \etal \cite{tomani2021towards} incorporated entropy-encouraging loss term with an adversarial calibration loss term to generate well-calibrated and trustworthy models. 



Generally, model calibration can be achieved through two methods: post-hoc calibration and calibration training.
%
Post-hoc calibration focuses on adjusting a model's output confidence as a post-processing step. Its main advantage is that it does not require updating or retraining the existing model. Zadrozny \etal \cite{zadrozny2001obtaining} first introduced histogram binning to produce calibrated probability estimates for decision tree and naive Bayesian classifiers. Subsequently, they proposed isotonic regression as a calibration technique \cite{zadrozny2002transforming}. Additionally, a more efficient and cost-effective post-hoc method is Platt Scaling \cite{platt1999probabilistic}, along with its single-parameter extension, Temperature Scaling, which has inspired various extensions \cite{mozafari2018attended,kull2019beyond,ding2021local}.
%
In terms of calibration training methods, Zhang \etal \cite{zhang2017mixup} proposed mixup regularization to create simple linear relationships between training examples. Tomani \etal \cite{tomani2021towards} introduced an entropy-encouraging loss term combined with an adversarial calibration loss term to develop well-calibrated and trustworthy models.


\subsection{Adversarial Attack}

% There are two settings of adversarial attacks. One is blackbox attack, refering that the attacker have rare information about the threaten models \cite{carlini2017towards}. And white-box attack means that the attacker has fully access to the target models \cite{goodfellow2014explaining}. One of the widely acknowledged defending method is adversarial training.
% Madry \etal \cite{madry2017towards} utilized adversarial examples as an augmentation during training to enhance the model's robustness.
% Stutz \etal \cite{stutz2020confidence} proposed Confidence-Calibrated Adversarial Training (CCAT) minimized the confidence of adversarial examples during training process to provide a sign to identify the attack cases, combining the low accurcy of the adversarial examples, generate a high calibration model against perturbation.
% By introducing an adversarial calibrated entropy term in training, Chen \etal \cite{chen2024integrating} also provide a limited confidence for perturbed input. 
%Combined with AT, it could generate higher accuracy than CCAT.

% Both CCAT and ACE address calibration issues during training by incorporating additional terms to mitigate them. However, they primarily focus on the overconfidence problem, overlooking the issue of underconfidence.
%
%In this work, we introduce underconfidence examples IAEs into the training process and 



There are two main settings for adversarial attacks. The first is the black-box attack, where the attacker has limited information about the target models \cite{carlini2017towards}. The second is the white-box attack, in which the attacker has full access to the target models \cite{goodfellow2014explaining}.
One widely recognized defense method is adversarial training. Madry \etal \cite{madry2017towards} employed adversarial examples as data augmentation during training to improve model robustness. Stutz \etal \cite{stutz2020confidence} introduced Confidence-Calibrated Adversarial Training (CCAT), which minimizes the confidence of adversarial examples during training to provide signals for identifying attack cases. Combined with the low accuracy of adversarial examples, this approach produces a highly calibrated model against perturbations. Similarly, Chen \etal \cite{chen2024integrating} proposed incorporating an adversarial-calibrated entropy term during training, which limits the confidence of perturbed inputs.

Both CCAT and ACE address calibration issues during training by incorporating additional terms. However, their focus is primarily on the overconfidence problem, often neglecting the issue of underconfidence.

==> misc/cvpr2025/sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> misc/cvpr2025/sec/3_method.tex <==
\section{Method}
\label{IAT:sec:method}
%In this section, we detailly introduce our Inverse adversarial attack and how we design the loss to satisfy the two conditions of underconfidence examples, including correctly predicted and limited confidence. Moreover, the framework of the defending method, \ie, Inverse Adversarial Training, is also Elaborated.
In this section, we provide a detailed introduction to our Inverse Adversarial Attack, outlining the design of the loss function to meet the two conditions for underconfidence examples: \textbf{correct prediction} and \textbf{limited confidence}. Furthermore, we elaborate on the framework of the defense method, \ie, Inverse Adversarial Training.


\subsection{Inverse Adversarial Attack}

% A perturbation $\N$ is inevitable during the storage or transfer of the multimedia data. Consequently, any input image, $\hat{\X}$, can be viewed as a combination of clear input $\X$ and $\N$.
A perturbation $\N$ is inevitable during the storage or transfer of multimedia data. Consequently, any input image, $\hat{\X}$, can be regarded as a combination of the clear input $\X$ and the perturbation $\N$:
\begin{align}\label{IAT:eq:addperturb}
\AE = \X + \N.         
\end{align}

%The differentiation degree decreases with the noise level of $\N$ increase. 
%对我们人类来说。一个input的辨识度会随着noise等级的增加而降低。我们对识别结果的准确率和信心都会下降。
%然而前面的介绍表示虽然model的准确率会随着noise的增加而下降 但是model对识别结果（尤其是错误的）会给予过高的信心。于是我们提出一个新颖的任务，他的目标是找出噪声图N，在混淆人类识别结果的同时获得model高置信度，以此来揭示人类与AI的矛盾。
%For humans, the recognizability of an input decreases as the level of noise increases, leading to reduced accuracy and confidence in the recognition results.
%As shown in \cref{IAT:fig:cover}, the accuracy of a well-trained model drops with noise increase, but it tends to produce predictions with over-high confidence for such noisy inputs.
%To address this discrepancy between human and AI perception, we propose a novel task: identifying noise maps 
%$\N$ that are confusing to human recognition but get high-confidence predictions from the model. This approach aims to reveal the inherent conflicts between human cognition and AI performance. 
%由于这个目的一半（over-confidence）与adversarial attack类似，而另一半(under-confidence)与之相反，所以我们称之为Calibration Attack
%inverse adversarial attack
%Since one aspect of this objective (over-confidence) is similar to adversarial attacks,  we refer to it as \textit{Calibration Adversarial Attack} (CAA).
%The other aspect (under-confidence) is the opposite, thus, we refer to it as \textit{Calibration Inverse Adversarial Attack} (CIAA).

%其中

%The targets of the CAA and CIAA are to generate the specific noise $\N$, which makes the model $\F(\cdot)$ outputs the highest maximum confidence while wrongly predicting or outputs the lowest maximum confidence while correctly predicting :
The objective of IAA is to generate specific noise $\N$, which causes the model $\F(\cdot)$ to output the lowest maximum confidence while making a correct prediction:
%over-confident example
%under-confident example：接近decision boundary
%体现出 哪些类与GT更相近，decision boundary更模糊

% \if 0
% %IAA
% \begin{align}
% \label{IAT:eq:IAA}
% %N = \mathop{\mathrm{argmax}}\limits_{\N}  ( MMC(\F(\X+\N))), s.t.~~\|\N\|_{\infty} \geq \epsilon,\\
% N = 
% \begin{cases} 
% &\mathop{\mathrm{argmax}}\limits_{N} (\text{MMC}(\F(\X+\N))), \\& \text{if } L(\F(\X+\N)) \neq \G\\
% &\mathop{\mathrm{argmin}}\limits_{N} (\text{MMC}(\F(\X+\N))), \\& \text{if } L(\F(\X+\N)) = \G \\
% \end{cases}
% s.t.~~\|\N\|_{\infty} \leq \epsilon,
% \end{align}
% \fi

% %IAE
% \begin{align}
% \label{IAT:eq:IAE_define}
% N = 
% \begin{cases} 
% &\mathop{\mathrm{argmax}}\limits_{N} (max(\F(\X+\N))), \\& \text{if } Label(\F(\X+\N)) \neq \G\\
% &\mathop{\mathrm{argmin}}\limits_{N} (max(\F(\X+\N))), \\& \text{if } Label(\F(\X+\N)) = \G \\
% \end{cases}
% s.t.~~\|\N\|_{\infty} \leq \epsilon,
% \end{align}

%IAE
\begin{equation}
\label{IAT:eq:IAE_define} 
\begin{aligned}
N = 
&\mathop{\mathrm{argmin}}\limits_{N} (max(\F(\X+\N))), \\
& s.t.~~ Label(\F(\X+\N)) = \G \\
& s.t.~~\|\N\|_{\infty} \leq \epsilon,
\end{aligned}
\end{equation}
where $Label(\cdot)$ means the predicted label of input. 
Since this objective (under-confidence) is opposite to adversarial attacks, we refer to it as \textit{Inverse Adversarial Attack} (IAA).
To jointly optimize the condition and object, we utilize the loss function for recognition, \eg, cross entropy loss, to replace $Label(\cdot)$ and $\mathop{\mathrm{argmin}}\limits_{N}(\cdot)$. Thus, the \cref{IAT:eq:IAE_define} is modified to:

%AE&IAE
\begin{equation}
\begin{aligned}
\mathcal{L}(\theta, &\X, \N, \G) =\\
%&\mathcal{L}_{CE}(\F(\X+\N), \G) - \lambda * \mathcal{L}_{EN}(\F(\X+\N))\\
&\mathcal{L}_{CE}(\F(\X+\N), \G) +  \lambda * \mathcal{L}_{CE}(\F(\X+\N), 1/K )
\end{aligned}
\label{IAT:eq:IAE2}
\end{equation}




% where $\text{MMC}(\cdot)$ refers to mean maximum confidence function. $\epsilon$ is the maximum perturbation. $L(\cdot)$ means the predicted label of input. To joint optimize the condition and object, we utilize a loss function for recognition, \eg, cross entropy loss, to replace $L(\cdot)$ and the \cref{IAT:eq:IAA} is modified to:

where $\mathcal{L}_{CE}(\cdot, \cdot)$ refers to cross entropy loss.  $\epsilon$ is the maximum perturbation. The first term guarantees a correct prediction result and the second term affects the prediction confidence. $\lambda$ controls the weight between two conditions.
By minimizes the $\mathcal{L}$, IAA provides the underconfident Inverse Adversarial Examples (IAEs):



%IAE
% \begin{align}
% \label{IAT:eq:N-AE}
% N_\mathrm{{CAE}} = &\mathop\mathrm{argmax}\limits_{N} \mathcal{L}
% \end{align}
\begin{align}
\label{IAT:eq:N-IAE}
N_{\mathrm{IAE}} = &\mathop\mathrm{argmin}\limits_{N} \mathcal{L}
\end{align}



% f(p)的图像展示与分析
%---------------------------
\begin{figure}[t]
\centering
        \centering
        \includegraphics[width=1\linewidth]{./figure/method/Lanalyze.pdf}
        \caption{The analysis of $\mathcal{L}$ in \cref{IAA:eq:optim} with $\lambda=5,~K=10$. $\mathcal{L}$ reaches its minimum when $y_G = 0.25$.}    
\label{IAA:fig:fp}
% \vspace{-4mm}
\end{figure}
%---------------------------


% Due to issues with ReLU network~\cite{hein2019relu}, the plain trained model exhibits overconfidence in the image space, particularly in areas far from the data distribution. As guidance, we propose a perturbation to provide the minimum confidence that the model can offer under a specific level of noise. Thus, we term this perturbation Minimum Confidence (MC). Its loss function is defined as follow:
% %minimum confidence
% \begin{align}
% \label{IAT:eq:MC}
% \mathcal{L}_{MC}(\theta, \X, \N) &= \mathcal{L}_{CE}(\F(\X+\N), 1/K )\\
% N_{MC} &= \mathop \mathrm{argmin}\limits_{N}\mathcal{L}_{MC}
% \end{align}

% \begin{align}
% \label{IAT:eq:IAA_2}
% \begin{split}
% &N = \mathop{\mathrm{argmax}}\limits_{N} (g(\theta,\X,\N,\G))\\
% &N = \mathop{\mathrm{argmin}}\limits_{N} (g(\theta,\X,\N,\G))\\
% &g(\theta,\X,\N,\G) = (\ell(\F(\X+\N) , \G) + \text{MMC}(\F(\X+\N)))\\
% &s.t.~~\|\N\|_{\infty} \leq \epsilon,
% \end{split}
% \end{align}

%its ground truth label $\G$, we usually minimize the energy function during the plain training process of:



Generally, we solve \cref{IAT:eq:N-IAE} by sign gradient descent. Note the number of attack iteration as $T$, and each pixel value in $\N$ is updated for every iteration $t$:

\begin{align}\label{IAA:eq:advupdate}
\N_{t} = \N_{t-1}~ - ~ \alpha~ \mathrm{sign}(\nabla \mathcal{L}_{\N_{t-1}}),
\end{align}
where $\alpha$ is the step size of each iteration. $\mathrm{sign}(\cdot)$ represents the signum function. $\nabla \mathcal{L}_{\N_{t-1}}$ denotes the gradient of $\N_{t-1}$ with respect to the objective function. 


%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%


\subsection{Optimization Analysis}
\label{IAA:subsec:optim}
Taken an input image, we note $y_k$ as the predict confidence of class $k$ along with classifier $\F$ and the entire predict distribution is $\mathbf{y} = \{y_1, y_2,...,y_K\}$. $K$ is the number of classes.
Let \( G \) be the ground truth label, and \( \mathbf{\hat{y}} \) be the one-hot representation of the ground truth, defined as:
\begin{equation}
\label{IAA:eq:y_hat}
\mathbf{\hat{y}} = 
\begin{cases}
\hat{y}_k = 1, & \text{if } k = G; \\
\hat{y}_k = 0, & \text{otherwise}.
\end{cases}
\end{equation}
Usually, the constrain of the $\sum_{k=1}^{K} y_k = 1$ is guaranteed by the final softmax layer $s(\cdot)$. 
Let's note $\mathbf{z}=\{z_k,k=1,2,...,K\}$ as the output logits before the final softmax layer, \ie, $ \mathbf{y} = s(\mathbf{z})$.
Moreover, we denote the uniform distribution $\mathbf{y^U}$ as $\{y^U_k = 1/K, i=1,2,...,K\}$.
Then, according to the definition of cross entropy, the loss function \cref{IAT:eq:IAE2} is reformulated as:



% \begin{align}\label{IAA:eq:optim}
% \mathcal{L} &= -log(p_{\G}) - \lambda * \frac{1}{K} \sum_{k=1}^{K} log(p_k),\\
% \mathcal{L} &= -(1+\frac{\lambda}{K})log(p_{\G}) - \lambda * \frac{1}{K} \sum_{k \neq \G} log(p_k),
% \end{align}
% where $p_{\G}$ refers to the predict confidence of Ground Truth label. $log(\cdot)$ means the logarithmic function. 
\begin{equation}
\begin{aligned}\label{IAA:eq:optim}
\mathcal{L} &= \mathcal{L}_{CE}(\mathbf{y},\mathbf{\hat{y}}) + \lambda * \mathcal{L}_{CE}(\mathbf{y},\mathbf{y^U}),
\end{aligned}
\end{equation}

where
As $z_k$ can be treated as individual, we then differentiate $\mathcal{L}$ with respect to $z_k$:
\begin{equation}
\begin{aligned}\label{IAA:eq:optim_dif}
\frac{\partial \mathcal{L}}{\partial z_k} 
&= \frac{\mathcal{L}_{CE}(\mathbf{y},\mathbf{\hat{y}})}{\partial z_k} +  \lambda * \frac{\mathcal{L}_{CE}(\mathbf{y},\mathbf{y^U})}{\partial z_k}\\
%&= \sum_{i=1}^{K}\frac{\mathcal{L}_{CE}(\mathbf{y},\mathbf{\hat{y}})}{\partial y_i}\frac{\partial y_i}{\partial z_k} +  \lambda * \sum_{i=1}^{K} \frac{\mathcal{L}_{CE}(\mathbf{y},\mathbf{y^U})}{\partial y_i}\frac{\partial y_i}{\partial z_k}\\
%&= \sum_{i=1}^{K}-\frac{\hat{y}_i}{y_i}\frac{\partial y_i}{\partial z_k} +  \lambda * \sum_{i=1}^{K} -\frac{y^U_i}{y_i}\frac{\partial y_i}{\partial z_k}\\
&= y_k-\hat{y}_k + \lambda * (y_k - y^U_k)\\
&= (1+\lambda)*y_k - (\hat{y}_k + \lambda * y^U_k)
\end{aligned}
\end{equation}

As $\lambda>0$, $1+\lambda>0$,  indicating that $\mathcal{L}$ is a concave function. Moreover, its minimum is attained under the condition:
\begin{equation}
\begin{aligned}\label{IAA:eq:optim_dif_k}
\frac{\partial L}{\partial z_k} &=0\\
(1+\lambda)*y_k - (\hat{y}_k + \lambda * y^U_k)&=0\\
y_k &=\frac{\hat{y}_k + \lambda * y^U_k}{1+\lambda}\\
\end{aligned}
\end{equation}

Finally, substituting \cref{IAA:eq:y_hat} yields:
\begin{equation}
\label{IAA:eq:optim_yk}
y_k = 
\begin{cases}
\dfrac{1 + \lambda / K}{1+\lambda}, & \text{if } k = G; \\
\dfrac{\lambda / K}{1+\lambda}, & \text{otherwise}.
\end{cases}
\end{equation}

%\cref{IAA:fig:fp} illustrates the relationship between $\mathcal{L}$ and predict probability $y_{G}$ along with model $\F$ when $\lambda = 5$ and $K=10$. 
%The figure indicates that the loss $\mathcal{L}$ reaches its minimum at $y_G = 0.25$, which demonstrates the correction of previous proof. 


In \cref{IAA:fig:fp}, we generate a curve to better illustrate the relationship between $\mathcal{L}$ and the predicted probability $y_{G}$, along with the model $\F$, when $\lambda = 5$ and $K=10$. The figure shows that the loss $\mathcal{L}$ reaches its minimum at $y_G = 0.25$, which is consistent with the previous analysis.

As $y_G - y_k|_{k \neq G}  = \dfrac{1}{1+\lambda} > 0$, the generated example should always be correctly classified, thereby meeting the first underconfidence criterion. Furthermore, its confidence level should be $y_G$ and negatively correlated with $\lambda$. Since the second condition requires minimizing confidence as much as possible, ideally, $\lambda$ should be maximized. However, considering implementation limitations, we can only approximate the optimization and cannot guarantee reaching it, so a certain margin between $y_G$ and $y_k$ is necessary. 
As $y_G - y_k= \dfrac{1}{1+\lambda}$ is inversely related to $\lambda$, we need to select a smaller $\lambda$ to ensure classification accuracy.
Given the conflicting requirements for $\lambda$, we conduct an experiment, and the results are presented in the next section to identify a trade-off between these two conditions for underconfidence examples.

% For the ground truth label $k=G$:
% \begin{equation}
% \begin{aligned}\label{IAA:eq:optim_dif_G}
% \frac{\partial L}{\partial z_G} 
% &= (1+\lambda)y_G - (\hat{y}_G + \lambda * y^U_G)\\
% &= (1+\lambda)y_G - (1 + \lambda * 1/K)\\
% \end{aligned}
% \end{equation}


%Then, $\mathcal{L}$ reaches the minimum point at $\frac{\partial L}{\partial z_G} =0$, \ie, $y_G= \frac{(1 + \lambda * 1/K)}{1+\lambda}$.


%
%Let the value of $y$ at which the loss $\mathcal{L}$ reaches its minimum be denoted as $y_{min}=\mathop \mathrm{argmin}\limits_{p}\mathcal{L}$. 
%

%Larger $\lambda$ generates lower confidence but likely affects the accuracy. To find a trade-off between these two conditions of underconfidence examples, we conduct an experiment and list the result in the next section.
%A larger $\lambda$ results in lower confidence but may impact accuracy. To balance these two conditions for underconfidence examples, we conduct an experiment, with the results presented in the next section.

% If $y_G>y_{min}$ $N_\mathrm{{CAE}}$ provides an example that is correctly predicted with high confidence. This is opposite to the definition of CAE. Applying small $\lambda (< 1)$ can increase the $p$ reaching the minimum point. However, this strategy reduces the effect of the second term and finally affects the confidence of CAE. As a result, an alternative way is proposed to avoid the problem. Concretely, we use $\mathcal{L}_{1}$ in the region where $p>p_{min}$ and $\mathcal{L}$ in the region where 
% $p \leq p_{min}$ to ensure the update direction of 
% $p$ is always negative:\
% %two stage function 
% \begin{align}
% \label{IAT:eq:l1}
% \mathcal{L}_{1}(\theta, \X, \N, \G) =\mathcal{L}_{CE}(\F(\X+\N), \G)
% \end{align}
% And apply the entire $\mathcal{L}$ for the rest iterations.
%
%In the meantime, we find that higher $\lambda$ causes the $p$ that minimizes
%$\mathcal{L}$ to approach $1/K$. However, as the minimization problem of \cref{IAT:eq:N-IAE} is approximately solved during the implementation, the accuracy of CIAE is hard to guarantee in that case. Similar to the strategy of CAE generation, we apply the second term in the first half iteration:
% \begin{align}
% \label{IAT:eq:l2}
% \mathcal{L}_{2}(\theta, \X, \N) = \mathcal{L}_{CE}(\F(\X+\N), 1/K )
% \end{align}
% Afterwards, the entire $\mathcal{L}$ is used for the rest updated.

%
Finally, by solving~\cref{IAA:eq:advupdate}, we generate the IAEs with the highest potential for revealing the contradiction between classification result and confidence. These examples serves as an augmentation during training to enhance the calibration of the DNN model. 
%\footnote{In the experiment, we choose $\alpha = 2 * \epsilon / T$.}
%
The specified step of generating IAEs is listed in \cref{IAA:alg:IAE}.

%pseudocode
% \begin{algorithm}
% \caption{Generate  CAE}\label{IAA:alg:AE}
% \begin{algorithmic}
% \State $\X \gets clear~input$
% \State $\N_0 \gets random~map$
% %\State $\AE \gets (\X+\N)$
% \State $\G \gets ground~truth~label$
% \State $p_{min} \gets \mathop\mathrm{argmin}\limits_{p} \mathcal{L}$
% \State $\epsilon \gets maximum~perturbation$
% \State $T \gets iteration~number$
% \State $t \gets 1$
% \State $\alpha \gets \epsilon / T$

% \While{$t \neq T$}

% \If{$p\geq p_{min}$} 
% \State $l \gets \mathcal{L}_{1}$
% \Else
% \State $l \gets \mathcal{L}(\theta,\X,\N_{t-1},\G)$
% \EndIf
% \State $grad \gets \mathrm{sign}(\nabla l_{\N_{t-1}})$
% \State $\N_{t} \gets \N_{t-1} ~+~\alpha * grad$
% \State $\N_{t} \gets \|\N_{t}\|_{\infty} \leq t*\epsilon / T$
% \State $t=t+1$
% \EndWhile
% \end{algorithmic}
% \end{algorithm}


\begin{algorithm}
\caption{Inverse Adversarial Attack}\label{IAA:alg:IAE}
\begin{algorithmic}
\State \textbf{Input:}
\State $\X \gets clear~input$
\State $\N_0 \gets random~map$
%\State $\AE \gets (\X+\N)$
\State $\G \gets ground~truth~label$
\State $\epsilon \gets maximum~perturbation$
\State $T \gets iteration~number$
\State $t \gets 1$
\State $\alpha \gets \epsilon / T$
\State \textbf{Output}: Inverse adversarial examples

\While{$t \neq T$}
\State $l \gets \mathcal{L}(\theta,\X,\N_{t-1},\G)$
\State $grad \gets \mathrm{sign}(\nabla l_{\N_{t-1}})$
\State $\N_{t} \gets \N_{t-1} ~-~\alpha * grad$
\State $\N_{t} \gets \|\N_{t}\|_{\infty} \leq t*\epsilon / T$
\State $t=t+1$
\EndWhile
\State return $\X+\N_T$
\end{algorithmic}
\end{algorithm}

% plot图展示IAE的效果


% framework
%---------------------------
\begin{figure*}[!th]
\centering
        \centering
        \includegraphics[width=.7\linewidth]{./figure/framework/framework.pdf}
        \caption{The framework of Inverse Adversarial Training.}    
\label{IAA:fig:framrwork}
% \vspace{-4mm}
\end{figure*}
%---------------------------



\subsection{Inverse adversarial Training}
\label{IAA:subsec:IAT}
The existence of IAEs demonstrates that the normally trained model may provide underconfidence prediction results. This may result in an unexpected reject problem (underconfidence) for an over-reliance AI model. For example, a self-driving system may have a delay response in recognizing sign on the expressway.
%a face recognition system may be cheated by a random mask, which may be unaware by the human guards.
%https://www.youtube.com/watch?v=_TXkDO5z11w
%person1 maybe detected as person2 with noisy mask

%
To avoid this phenomenon, we propose an \textit{Inverse Adversarial Training} (IAT), in which we add the IAEs in the training process. They use the capability of these examples to reveal the uncalibrated cases and enhance the model's calibration. The framework of our proposed training is illustrated in \cref{IAA:fig:framrwork}.




%
Usually, a plain training process is to optimize such a target function:
%plain trainig
\begin{align}
\label{IAT:eq:trainplain}
\mathop{\mathrm{min}}\limits_{\theta} \mathbb{E}_{(\X,\G) \sim \mathcal{D}} [\ell(\F(\X), \G)],
\end{align}
where ${\mathcal{D}}$ is the data distribution. The normal training process updates the parameters $\theta$ in the DNN model by minimizing the loss.

The target of IAT is to minimize the loss of uncalibrated examples. Different from Adversarial Training, which focus on increasing the accuracy of overconfident adversarial examples to guarantee the robustness of model, the IAT adjust the outputs of underconfident examples generated by models.
Thus, the objective function~\cref{IAT:eq:trainplain} is then modified with~\cref{IAT:eq:IAE2} for IAT:
% \begin{align}
% \label{IAT:eq:CAT}
% \mathbb{CAT}:~\mathop{\mathrm{min}}\limits_{\theta} \mathbb{E}_{(\X,\G) \sim \mathcal{D}} [\mathcal{L}_2(\theta, &\X, \mathop{\mathrm{argmax}}\limits_{\N \in \Omega}\mathcal{L})],
% \end{align}
\begin{align}
\label{IAT:eq:IAT}
\mathbb{IAT}:~\mathop{\mathrm{min}}\limits_{\theta} \mathbb{E}_{(\X,\G) \sim \mathcal{D}} [\ell(\F(\X+\mathop{\mathrm{argmin}}\limits_{\N \in \Omega}\mathcal{L}), \G)],
\end{align}
where $\Omega$ represents the perturbation space, which is $\|N\| \leq \epsilon$.
During the training phase, IAT incorporates IAEs into the model, addressing underconfidence cases.

In the implementation, IAT updates the model's parameters in $I$ times iteration. We first generate the noisy map $\N_0$ with the initial model $f_{\theta_0}$. Afterward, in each iteration $i$, we update the model's parameters $\theta_i$ according to the gradient descent:
\begin{align}\label{IAT:eq:optim_CAT}
\theta_{i} = \theta_{i-1} ~ - ~ \eta~ \nabla_{\theta} \ell(\theta_{i-1},\X,\N_{i-1},\G),
\end{align}
where $\eta$ refers to the learning rate.
%Generally, we want to use accuracy as a guidance to adjust the confidence of the model.




%where $\ell(\cdot , \cdot)$ refers to the loss function, \eg, cross entropy loss.


\if 0
To enhance the specificity of the model against noisy inputs, we utilize SSIM value to guide the output confidence during the training process and change the training function as follow:

%general specify enhancement training
\begin{align}
\label{IAT:eq:G_trainbaseline}
&\mathop{\mathrm{min}}\limits_{\theta} \mathbb{E}_{(\X,\G) \sim \mathcal{D}} [\ell(\F(\X), \G)\\ 
&+    \sum\limits_{i=1}^{I} MSE(MMC(\F(\X+\mathbf{\N}_i)) , g_{i}(\X+\mathbf{\N}_i))],
\end{align}
where $g_i(\cdot), i=1 \cdots I$ is a function set indicating the confidence model in different noise scales.

%这里 我们使用一个带阈值的曲线来表征，低噪声下需要更高的mmc来保证robustness， 高噪声下更低的mmc来体现specificity
In this paper, we utilize a threshold model 
%baseline(random noise) training
\begin{align}
\label{IAT:eq:trainbaseline}
\mathop{\mathrm{min}}\limits_{\theta} \mathbb{E}_{(\X,\G) \sim \mathcal{D}} [\ell(\F(\X), \G) +    MSE(MMC(\F(\textbf{N})) , SSIM(\textbf{N}))],
\end{align}


%IAD aug training
\begin{align}
\label{IAT:eq:trainIAD}
\mathop{\mathrm{min}}\limits_{\theta} \mathbb{E}_{(\X,\G) \sim \mathcal{D}} [\ell(\F(\X), \G) +    MSE(MMC(\F(\textbf{IAE})) , SSIM(\textbf{IAE}))],
\end{align}

%adv
\begin{align}
\label{IAT:eq:trainADV}
\mathop{\mathrm{min}}\limits_{\theta} \mathbb{E}_{(\X,\G) \sim \mathcal{D}} [\ell(\F(\X), \G) + \ell(\F(\textbf{ADE}), \G)],
\end{align}


%adv + baseline(random noise) training
\begin{align}
\label{IAT:eq:trainADVbaseline}
\mathop{\mathrm{min}}\limits_{\theta} \mathbb{E}_{(\X,\G) \sim \mathcal{D}} [\ell(\F(\X), \G) 
+   \ell(\F(\textbf{ADE}), \G)
+    MSE(MMC(\F(\textbf{N})) , SSIM(\textbf{N}))],
\end{align}


%adv + iad aug training
\begin{align}
\label{IAT:eq:trainADVIAD}
\mathop{\mathrm{min}}\limits_{\theta} \mathbb{E}_{(\X,\G) \sim \mathcal{D}} [\ell(\F(\X), \G) 
+   \ell(\F(\textbf{ADE}), \G)
+    MSE(MMC(\F(\textbf{IAE})) , SSIM(\textbf{IAE}))],
\end{align}

\fi

==> misc/cvpr2025/sec/4_experiments.tex <==
\section{Experiments}
\label{IAT:sec:exp}


% lambda of IAA
%---------------------------
\begin{figure*}[!th]
\centering
        \centering
        \begin{subfigure} {.32\textwidth}
        \includegraphics[width=1\linewidth]{./figure/lambda_tune/lambtuning_ACC.pdf}
        \caption{}
        \end{subfigure} 
        \begin{subfigure} {.32\textwidth}
        \includegraphics[width=1\linewidth]{./figure/lambda_tune/lambtuning_CONF.pdf}
        \caption{}
        \end{subfigure} 
        \begin{subfigure} {.32\textwidth}
        \includegraphics[width=1\linewidth]{./figure/lambda_tune/lambtuning_MCS.pdf}
        \caption{}
        \end{subfigure} 
        \caption{Apply different IAA with different $\lambda$ against to a well-trained model on CIFAR10. ACC, CONF and MCS are shown along with $\epsilon$ ranging from $0.02$ to $0.1$.}    
\label{IAA:fig:lambda_tune}
% \vspace{-4mm}
\end{figure*}
%---------------------------

%布里尔分数 Brier Score
%然而BS是对于clear input计算的，对于perturbation input的ground truth label（即是否能被人类正确识别）是一个主观的问题。所以我们

%MNIST, CIFAR10, CIFAR100, ImageNet.

\paragraph{Metric:}
\textbf{Accuracy (ACC)} represents the proportion of correctly predicted cases among all input images. \textbf{Confidence (CONF)} refers to the maximum value of the softmax output in the classifier network's final layer. Note that ``the confidence of the ground truth label'' refers to the probability assigned by a classifier to the ground truth label as its prediction.
As our work focuses more on the underconfidence problem, we choose \textbf{Miscalibration Score (MCS)} \cite{pmlr-v216-ao23a} as our metric to evaluate the calibration of a model during our experiments. Different with the widely-used Expected Calibration Error (ECE) \cite{guo2017calibration} that considers the inconformity of accuracy and confidence equally, MCS expresses overconfidence and underconfidence with the positive or negative value.
% ECE is defined by the prediction accuracy and confidence:
% \begin{align}
% \label{IAT:eq:ECE}
% ECE =  \sum_{m=1}^{M} \frac{|B_m|}{N} |acc(B_m)-conf(B_m)|,
% \end{align}
MCS is defined by the prediction accuracy and confidence:
\begin{align}
\label{IAT:eq:MCS}
MCS =  \sum_{m=1}^{M} \frac{|B_m|}{N} (acc(B_m)-conf(B_m)),
\end{align}
where $M$ is the number that separates the confidence range into several bins and $N$ indicates the total number of cases. Generally, MCS reflects the inconsistency between accuracy and confidence.
\textbf{Generally, an MCS value approaching $0$ indicates better model calibration. A higher absolute MCS value suggests a stronger ability of the attack to expose a model's miscalibration issues, where positive values indicate overconfidence and negative values indicate underconfidence.}

\if 0
naive Bayesian prediction possibility, $o_{i}$ represents the ground truth label. 
However, this definition is utilized for clear input. The ground truth label for a perturbation input, is a subjective problem. Consequently, we use correct classification (CC) function $cc_i$ to replace $o_i$:
\begin{align}
\label{IAT:eq:CC}
cc_i = \begin{cases}
 1, ~if~\AE_i~is~correctly~predicted\\
 0, ~if~\AE_i~is~wrongly~predicted\\
\end{cases}  ,
\end{align}
Then the \cref{IAT:eq:BrierScore} is reformulated as:
\begin{align}
\label{IAT:eq:BrierScore2}
BS = \frac{1}{N} \sum_{i=1}^{n}(p_i-cc_i)^2,
\end{align}

\fi

\paragraph{Datasets and Threaten models:} 
%For most experiments, we utilize ResNet18 as backbone of classifier. Our proposed IAT and AT+IAT models are evaluated with other models with several baselines training strategies including, plain training (PT), PGD adversarial training (PGD-AT) \cite{madry2017towards}, confidence-calibrated adversarial training (CCAT) \cite{stutz2020confidence}, adversarial calibration entropy enhanced training (ACE-AT) \cite{chen2024integrating}. Note that the AT strategy applied in AT+IAT is PGD-AT.
%Specifically, each training strategy is conducted with adam optimizer, and a learning rate of $0.01$.
%, reaching an accuracy of $87.93\%$ and a mean confidence of $96.12\%$.
%Moreover, we also apply IAA among PT models with different backbones, including ResNet18, MobileNet and VGG19, to evaluate the transferability of IAA.

%\paragraph{Baseline perturbation:} uniform noise (UN), PGD \cite{madry2017towards}.

 For most experiments, we use ResNet18 \cite{He2015DeepRL} as the backbone of the classifier. Our proposed IAT and AT+IAT models are evaluated alongside other models using several baseline training strategies, including plain training (PT), PGD adversarial training (PGD-AT) \cite{madry2017towards}, confidence-calibrated adversarial training (CCAT) \cite{stutz2020confidence}, and adversarial calibration entropy-enhanced training (ACE-AT) \cite{chen2024integrating}. It is important to note that the AT strategy applied in AT+IAT follows the PGD-AT method.
Most experiments are conducted on the CIFAR10 dataset \cite{krizhevsky2009learning}, with the exception of a qualitative analysis performed on the NeurIPS'17 adversarial competition dataset \cite{kurakin2018adversarial} using a pretrained VGG19 model \cite{simonyan2014very}.



\subsection{$\lambda$ evaluation}
%In this section, we evaluate the capability of revealing underconfidence issues with different $\lambda$. As mentioned in \cref{IAA:subsec:optim}, larger $\lambda$ provide lower confidence yet lower $\lambda$ guarantee the accuracy. Considering this, we apply IAA against a well-trained ResNet18 model on CIFAR10 dataset with different values of $\lambda$.  The result is shown in 
In this section, we evaluate the ability to reveal underconfidence issues using different values of $\lambda$. As discussed in \cref{IAA:subsec:optim}, larger values of $\lambda$ result in lower confidence, while smaller values help maintain accuracy. Based on this, we apply IAA to a well-trained ResNet18 model on the CIFAR-10 dataset with various $\lambda$ values. The results are shown in \cref{IAA:fig:lambda_tune}. 

We illustrate the ACC, CONF and MCS of IAA with different $\lambda=1, 3, 5, 7, 10$.
MCS is a signed score representing the miscalibration of a model. With a higher absolute value  the model is more miscalibrated.
\cref{IAA:fig:lambda_tune} (a) indicates that the ACC decreases with the increase of $\lambda$, which demonstrates our concern of safe margin for accuracy.
\cref{IAA:fig:lambda_tune} (b) illustrates the negative correlation between $\lambda$ and $y_G$ in minimization point of $\mathcal{L}$, which is consistent with our previous conclusion.
Referring to the MCS values in \cref{IAA:fig:lambda_tune} (c), we choose $\lambda = 5$ for IAA in the following experiments.
As a result, the $y_G=0.25$ with $K=10$ and $y_G=0.1675$ with $K=1000$.

%\yupeng{analysis acc conf mcs}







\subsection{Underconfidence issues for different backbones}
%因为模型训练需要时间，所以先按照model来分列图表。等都train好之后，再按照perturbation分类图表。在没有很多baseline的时候，这样更有说服力。
% plain trained model, AT, IAT, CCAT,ACE.
%To evaluate the capability of IAE in revealing the uncalibrated feature of a model, we conduct an experiment that compares the MCS of perturbed examples generated by all perturbation methods against each model. 


To illustrate the difference in calibration impact between AA and our IAA, we generate uniform noise (UN), PGD adversarial attacks (AA), and IAA with maximum perturbations ranging from $\epsilon = 0.02$ to $0.1$, and plot them along with their MCS. The result is shown in \cref{IAA:fig:MCS_eps_plain}.

%We can see that the MCS of UN (normalnoi) grows with the $\epsilon$ increases, indicating that the plain trained model exhibits overconfidence with higher perturbation.
%However, the capability of random noise in revealing the uncalibration is limited as it can rarely produce over-confidence examples with high MCS. 
It is evident that the MCS of UN increases as $\epsilon$ grows, indicating that the plain trained model exhibits increasing overconfidence with higher levels of perturbation. However, the effectiveness of uniform noise in exposing model miscalibration is limited, as it seldom generates overconfident examples with high MCS.
%In contrast, CAE (ae) could generate examples with high MCS even in a small perturbation. For example, the CAE reaches 0.85 MCS with a perturbation level $0.02$. 
In contrast, PGD adversarial attack (AA) is capable of generating examples with high MCS even under small perturbations. For instance, AA achieves an MCS of $0.85$ at a perturbation level of $0.02$.
%Note that, only CIAE is able to produce examples with nagative MCS. In another word, reveal the underconfidence of the PT model.

Notably, only IAA is capable of generating examples with negative MCS, thereby revealing the underconfidence issue of the PT model. 
The absolute value of AA exceeds that of IAA, suggesting that achieving overconfidence is easier than inducing underconfidence. 
This can be attributed to the fact that suppressing the softmax confidence for the ground truth label guarantees lower accuracy without conflicting with the increase in maximum softmax confidence. Conversely, reducing the maximum softmax confidence has a pronounced negative impact on accuracy.
%The reason is that overconfidence examples are generated by reducing accuracy, achieved by minimizing the confidence of the ground truth label, which does not conflict with increasing the maximum confidence. In contrast, underconfidence examples require boosting accuracy by maximizing the confidence of the ground truth label, which significantly conflicts with maintaining low confidence.
% MCS-epsilon plain
%---------------------------
\begin{figure}[!t]
\centering
        \centering
        \includegraphics[width=.8\linewidth]{./figure/perturb2PT/plain_MCS.pdf}
        \caption{MCS of the examples generated by uniform noise (UN), PGD attack (AA), IAA against to PT model with maximum perturbation $\epsilon$ ranging from $0.02$ to $0.1$. The red dot line indicates the perfect calibration, \ie, MCS=0.}    
\label{IAA:fig:MCS_eps_plain}
% \vspace{-4mm}
\end{figure}
%---------------------------

% \yupeng{accomplish if available...}
% Moreover, To showcase the effectiveness of IAA in revealing a model’s miscalibration features, we compare the MCS of IAEs crafted for models with various backbones, including ResNet18, MobileNet, VGG19 and InceptionV3.




% MCS-epsilon: IAA against to different models
%---------------------------
\begin{figure}[!th]
\centering
        \centering
        % \begin{subfigure} {.32\textwidth}
        % \includegraphics[width=1\linewidth]{./figure/IAA/difmodel_iae_ACC.pdf}
        % \caption{}
        % \end{subfigure}
        \begin{subfigure} {.4\textwidth}
        \includegraphics[width=1\linewidth]{./figure/IAA/difmodel_iae_MCS.pdf}
        \caption{}
        \end{subfigure}
        \begin{subfigure} {.4\textwidth}
        \includegraphics[width=1\linewidth]{./figure/IAA/difmodel_iae_CONF.pdf}
        \caption{}
        \end{subfigure}
        \caption{MCS and CONF of IAA against to PT, PGD-AT, ACE-AT, CCAT, IAT and AT+IAT models with maximum perturbation $\epsilon$ ranging from $0.02$ to $0.1$.}    
\label{IAA:fig:IAAquanti}
% \vspace{-4mm}
\end{figure}
%---------------------------

% MCS-epsilon: PGD against to different models
%---------------------------
\begin{figure*}[th]
\centering
        \centering\centering
        \begin{subfigure} {.32\textwidth}
        \includegraphics[width=1\linewidth]{./figure/PGD/difmodel_adv_ACC.pdf}
        \caption{}
        \end{subfigure}
        \begin{subfigure} {.32\textwidth}
        \includegraphics[width=1\linewidth]{./figure/PGD/difmodel_adv_CONF.pdf}
        \caption{}
        \end{subfigure}
        \begin{subfigure} {.32\textwidth}
        \includegraphics[width=1\linewidth]{./figure/PGD/difmodel_adv_MCS.pdf}
        \caption{}
        \end{subfigure}
        \caption{ACC, CONF and MCS of PGD attack against to PT, PGD-AT, ACE-AT, CCAT, IAT and AT+IAT models with maximum perturbation $\epsilon$ ranging from $0.02 \sim 0.1$.}    
\label{IAA:fig:PGD}
% \vspace{-4mm}
\end{figure*}
%---------------------------


\subsection{Quantitative Analysis of IAA}
To demonstrate the effectiveness of IAA in exposing underconfidence issues, we evaluate the MCS and CONF of IAEs crafted for models trained with various strategies, including PT, PGD-AT, ACE-AT, CCAT, IAT and AT+IAT.
%
%We compare the performance of IAA against to all baseline models based on the MCS along with maximum perturbation $\epsilon$ for a fair comparison.
%
Concretely, we vary the $\epsilon$ for different target models to generate multiple MCS-$\epsilon$ curves for clear visual comparison. The results are presented in \cref{IAA:fig:IAAquanti}. 

Generally, the PT model is affected by IAA, while calibrated adversarial training methods (CCAT and ACE-AT) are more sensitive to IAA as they only address the overconfidence issue by minimizing the confidence of any perturbation, as shown in \cref{IAA:fig:IAAquanti} (b).
%
% The PGD-AT shows some resistance to IAA, as it increases the minimum confidence in the $\epsilon$-neighborhood of the input image.
% Our IAT demonstrates the best performance in resisting IAA. 
% Moreover, the AT+IAT, integrating the IAEs and AEs into training process, showcases a similar resistance against to IAA, even better (low absolute MCS values) with low perturbation level ($\epsilon < 0.08$).
PGD-AT exhibits some resistance to IAA, as it increases the minimum confidence within the $\epsilon$-neighborhood of the input image. Our IAT achieves the best performance in resisting IAA. Furthermore, AT+IAT, which integrates IAEs and AEs into the training process, demonstrates comparable resistance to IAA and even better performance (lower absolute MCS values) at low perturbation levels ($\epsilon < 0.08$).
% accurate IAE generate better IAT

% In this section, we implement the CAT and CIAT metioned in \ref{IAA:subsec:ATIAT}, and evaluated their capability in defending the CAE and CIAE.
% Furthermore, we integrate CAT and CIAT to develop a calibration-enhanced training approach, referred to as Calibrated Training (CT).


\subsection{Quantitative Analysis of PGD attack}
In this part, we evaluate the robustness of IAT and AT+IAT in resisting overconfidence attack.
Specifically, we apply the PGD attack against to all baseline models and our proposed IAT and AT+IAT models with a sliding maximum perturbation $\epsilon$ ranging from $0.02$ to $0.1$.
The results are shown in \cref{IAA:fig:PGD}

%acc
As shown in \cref{IAA:fig:PGD} (a), although PGD-AT and ACE-AT maintain the highest robustness, IAT can still partially resist PGD (overconfidence) attacks, even as an underconfidence defense method that has not encountered any adversarial examples during training.
%conf
Moreover, both PGD-AT and ACE-AT sacrifice confidence to achieve greater robustness, which makes the models more risk-averse.
%mcs
Besides, with respect to MCS, IAT also shows some resistance compared to PT. PGD-AT demonstrates significant resistance to PGD attacks since it is exposed to PGD examples during training. Note that ACE-AT exhibits an underconfidence phenomenon, as it minimizes confidence to an extremely low level. CCAT achieves the best MCS values (approaching $0$) by minimizing confidence under varying levels of noise, regardless of their accuracy.
Finally, AT+IAT achieves the same level of robustness as PGD-AT while also demonstrating good calibration under IAA. Its strong performance in resisting IAA suggests that combining AT and IAT is an effective approach for producing a well-calibrated model capable of withstanding both overconfidence attacks (\eg, AA) and underconfidence attacks (\eg, IAA).



%---------------------------
\begin{figure*}[!th]
\centering
        \centering
        \includegraphics[width=.9\linewidth]{./figure/visualization/visualization.pdf}
        \caption{Visualization of inverse adversarial examples generated for the VGG19 network pretrained on ImageNet. Clear input images (wrongly predicted by the pretrained model) are shown in the first row, with IAEs displayed in the second row. Each image displays its classification result from VGG19 in the top-left corner. The predicted confidence levels are shown at the bottom. Incorrect predictions are highlighted in red and correct predictions are highlighted in green.}    
\label{IAA:fig:visual}
% \vspace{-4mm}
\end{figure*}
%---------------------------





%---------------------------
%---------------------------Qualitative


\subsection{Qualitative Analysis of IAA}
\yupeng{add acc-conf plot (calibration histogram) in the figure}
To visually demonstrate the effectiveness of IAA, we conduct an experiment on a high-resolution image dataset from the NeurIPS'17 adversarial competition, specifically the DEV dataset \cite{kurakin2018adversarial}, which is compatible with ImageNet \cite{deng2009imagenet}. We use a VGG19 network pretrained on ImageNet as the threaten model. In this experiment, we set the maximum IAA perturbation $\epsilon$ to $0.03$. The clear input images and corresponding IAEs are shown in \cref{IAA:fig:visual}.

Given that the 1000-class classification task is highly challenging, the top-1 accuracy of this pretrained VGG19 on the NeurIPS2017 dataset only reaches $87.6\%$, resulting in some misclassified cases. For example, the image in the second column is incorrectly predicted as 'water tower' with a high confidence of $67.2\%$, indicating overconfidence in this instance\yupeng{refer a average confidence here}. The reason could be that, from this angle, the mosque indeed bears some resemblance to a water tower. Similar situations also occur in the case shown in the third column.
However, IAA successfully generates examples with correct predictions but lower confidence (e.g., $4.7\%$ for the ambiguous second case) using imperceptible perturbations. This demonstrates that our proposed IAA effectively reveals potential underconfidence issues even in cases prone to confusion.


%The five clear inputs (1st column) are wrongly classified, and IAEs can be correctly predicted with limited confidence.
% visualization



\subsection{Discussion on Transferability of IAA}

\begin{table}[h!]
\centering

\resizebox{0.45\textwidth}{!}{
\begin{tabular}{|c|c|c|c|}
    \hline
    \diagbox{Target}{Threaten} & ResNet18 & MobileNet & VGG19 \\ \hline
    ResNet18 & -0.6887 & 0.0234 & 0.0313 \\ \hline
    MobileNet & 0.0703 & -0.7192 & 0.0415 \\ \hline
    VGG19 & 0.0664 & 0.0153 & -0.2395 \\ \hline
\end{tabular}
}
\caption{We present the MCS results of transfer and white-box inverse adversarial attacks across three fine-tuned models: ResNet18, MobileNet, and VGG19. The whitebox attack results are shown along the diagonal, while the remaining results correspond to transfer attacks.}
\label{IAA:tab:transferability}
\end{table}

Transferability refers to the ability of an attack to successfully affect a target model using examples generated from a different threaten model. Evaluating the transferability of IAA is important, as it aligns more closely with real-world attack scenarios.
%
To investigate the transferability of IAA, we apply IAA on three well-trained threaten models, including ResNet18, MobileNet and VGG19, to generate corresponding IAEs with a maximum perturbation of $\epsilon=0.03$. These IAEs are then fed back to the models as target models, yielding nine MCS values that reflect the impact of IAA on each.
%
Following terminology from the adversarial attack field, when the threaten model and target model are identical, we refer to this as a ``whitebox'' IAA, indicating full access to the target model. Conversely, when the threaten model and target model differ, we refer to it as ``transfer'' IAA.

\cref{IAA:tab:transferability} presents the MCS results for transfer and whitebox IAAs across three fine-tuned models: ResNet18, MobileNet, and VGG19. In the table we have the following observation:

Diagonal entries (\eg, ResNet18-ResNet18) represent the whitebox IAA results, indicating the attack performance on each model’s own architecture is significant.
Specifically, the whitebox IAA against to ResNet18 has a MCS value of $-0.6887$, showing a strong reduction in model calibration under attack.
Same phenonmenon exists to the MobileNet.
The MCS value of whitebox IAA against to VGG19 is $-0.2395$, which, though higher (lower in absolute value) than that of ResNet18 and MobileNet, still shows a substantial impact on calibration by whitebox IAA.

%Off-diagonal entries represent transfer attack results. The results shows that changing architecture of model has huge effect to the effectiveness of IAA. For instance, VGG19’s attacks on ResNet18 and MobileNet yield MCS values of $0.0664$ and $0.0153$, respectively.
Off-diagonal entries represent transfer attack results. The findings indicate that changing the model architecture significantly affects the effectiveness of IAA. For instance, IAEs crafted from VGG19 yield MCS values of $0.0664$ and $0.0153$ when attacking ResNet18 and MobileNet, respectively.

%In summary, the whitebox IAA generally produces large negative MCS values, indicating a notable capability of revealing underconfidence issues. In contrast, the transfer IAA tends to have MCS values close to zero or even positive, suggesting lower effectiveness, making enhance the transferability of IAA be a proteintal topic as a future work.
In summary, whitebox IAA typically produces large negative MCS values, highlighting its strong ability to expose underconfidence issues. In contrast, transfer IAA generally yields MCS values closer to zero or even positive, indicating lower effectiveness. Enhancing the transferability of IAA presents a promising direction for future research.


==> misc/cvpr2025/sec/5_conclusion.tex <==
\section{Conclusion}
\label{IAT:sec:conclusion}
% Calibration is a very important feature in the reliable AI system. recent works mostly focus on dealing with the overconfidence problem, \eg, adversarial attack.
% In this paper, we explored the other side of miscalibration by proposing a novel task that generates correctly predicted examples with minimum confidence, termed as \textit{Inverse Adversarial Attack}.
% To meet the two conditions of underconfidence, correct prediction and limited confidence, we integrated two cross-entropy loss to provide a trade-off in generating the inverse adversarial examples.
% We then mathematically analyzed the proposed loss function and proved that the minimization of it can fulfill the two conditions of underconfidence.
% Substantial experimental results showed that our IAA can effectively reveal the underconfidence issue and can be embedded into the training process, which called IAT, to resist such attack. Combining the AT and IAT is practical and provide a model that simultaneously robust and calibrated.
Calibration is a crucial feature for reliable AI systems. Recent work has primarily focused on addressing the issue of overconfidence, such as through adversarial attacks. In this paper, we explore the opposite side of miscalibration by proposing a novel task that generates correctly predicted examples with minimal confidence, termed the Inverse Adversarial Attack (IAA). To satisfy the two conditions of underconfidence—correct prediction and low confidence—we incorporate two cross-entropy loss terms to balance the trade-off in generating inverse adversarial examples. We then provide a mathematical analysis of the proposed loss function, demonstrating that its minimization meets the two conditions of underconfidence.
Extensive experimental results show that our IAA effectively reveals underconfidence issues and can be embedded in the training process, forming what we term Inverse Adversarial Training (IAT) to counter such attacks. Combining adversarial training (AT) with IAT provides a practical approach to achieve models that are both robust and well-calibrated.
Additionally, the discussion on the transferability of IAA provides a potential direction for future work.
